Generating Information-Seeking Conversations from Unlabeled Documents

In this paper, we introduce a novel framework, SIMSEEK, (Simulating information-Seeking conversation from unlabeled documents), and compare its two variants. In our baseline SIMSEEK-SYM, a questioner generates follow-up questions upon the predetermined answer by an answerer. On the contrary, SIMSEEK-ASYM first generates the question and then finds its corresponding answer under the conversational context. Our experiments show that they can synthesize effective training resources for CQA and conversational search tasks. As a result, conversations from SIMSEEK-ASYM not only make more improvements in our experiments but also are favorably reviewed in a human evaluation. We finally release a large-scale resource of synthetic conversations, WIKI-SIMSEEK, containing 2 million CQA pairs built upon Wikipedia documents. With the dataset, our CQA model achieves state-of-the-art performance on a recent CQA benchmark, QuAC.

==> archive/human_eval_orig.tex <==
\begin{table*}[t!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|l|ccc|ccc|ccc|ccc|ccc}
    \toprule
    \multirow{2}{*}{Dataset} & \multirow{2}{*}{Evaluation Pair} & \multicolumn{3}{c|}{Overall} & \multicolumn{3}{c|}{Informativeness} & \multicolumn{3}{c|}{Context Relevance} & \multicolumn{3}{c|}{Answer-Specificity} & \multicolumn{3}{c}{Answer Accuracy} \\
     & & higher & neutral & lower & higher & neutral & lower & higher & neutral & lower & higher & neutral & lower & higher & neutral & lower \\
     \midrule
     \multirow{3}{*}{All} & asym-sym & 0.37 & 0.21 & \textbf{0.41} & 0.37 & 0.22 & \textbf{0.41} & 0.35 & 0.22 & \textbf{0.43} & 0.36 & 0.19 & \textbf{0.45} & 0.34 & 0.20 & \textbf{0.46} \\
     & asym-human & \textbf{0.48} & 0.13 & 0.39 & 0.39 & 0.19 & \textbf{0.42} & 0.38 & 0.23 & 0.38 & 0.40 & 0.16 & \textbf{0.44} & \textbf{0.38} & 0.28 & 0.34  \\
     & sym-human & \textbf{0.42} & 0.17 & 0.41 & \textbf{0.46} & 0.20 & 0.35 & \textbf{0.46} & 0.19 & 0.35 & \textbf{0.48} & 0.15 & 0.37 & \textbf{0.44} & 0.20 & 0.36 \\
     \midrule
     \multirow{3}{*}{Answerable} & asym-sym & 0.38 & 0.22 & \textbf{0.40} & 0.39 & 0.20 & \textbf{0.41} & 0.35 & 0.23 & \textbf{0.42} & \textbf{0.41} & 0.20 & 0.39 & 0.36 & 0.19 & \textbf{0.45} \\
     & asym-human & \textbf{0.49} & 0.13 & 0.38 & 0.39 & 0.18 & \textbf{0.43} & \textbf{0.37} & 0.27 & 0.36 & 0.37 & 0.14 & \textbf{0.49} & 0.34 & 0.32 & 0.34 \\
     & sym-human & 0.39 & 0.16 & \textbf{0.45} & \textbf{0.41} & 0.20 & 0.39 & \textbf{0.46} & 0.18 & 0.36 & \textbf{0.43} & 0.15 & 0.41 & \textbf{0.40} & 0.22 & 0.39 \\
     \midrule
     \multirow{3}{*}{Filtered} & asym-sym & \textbf{0.42} & 0.23 & 0.34 & 0.40 & 0.17 & \textbf{0.42} & 0.37 & 0.18 & \textbf{0.43} & \textbf{0.40} & 0.21 & 0.39 & 0.34 & 0.20 & \textbf{0.44} \\
     & asym-human & \textbf{0.49} & 0.13 & 0.37 & 0.40 & 0.17 & \textbf{0.43} & \textbf{0.39} & 0.27 & 0.34 & 0.37 & 0.13 & \textbf{0.50} & 0.36 & 0.28 & \textbf{0.37} \\
     & sym-human & 0.36 & 0.17 & \textbf{0.47} & \textbf{0.43} & 0.18 & 0.39 & \textbf{0.47} & 0.21 & 0.33 & \textbf{0.45} & 0.16 & 0.39 & 0.38 & 0.23 & 0.38 \\
    \bottomrule
\end{tabular}}
\caption{Pairwise human evaluation results for the original QuAC (human) and the synthetic conversations from \textsc{SimSeek} (sym and asym). 
Given the same conversation and documents, the annotators are asked to pick the better one in the criterion from two random QA pairs.
Since the bias of annotators on unanswerable and ``Anything else?'' questions, we filtered them out (Filtered) when evaluating conversations.
We show the percentage of majority votes for each criterion.
}
\label{table:case_study}
\vspace{-.4cm}
\end{table*}

==> archive/unseen_old.tex <==
\begin{table*}[t!]
    \centering
    \begin{threeparttable}
    \begin{tabular}{l|cc|cc|cc}
        \toprule
        Synthetic CQA & \multicolumn{2}{c|}{RoBERTa-base} &  \multicolumn{2}{c|}{RoBERTa-large}  & \multicolumn{2}{c}{Longformer-large} \\
        Generation & $\hat{\mathcal{D}}$ & $\mathcal{D}$ + $\hat{\mathcal{D}}$ & $\hat{\mathcal{D}}$ & $\mathcal{D}$ + $\hat{\mathcal{D}}$ & $\hat{\mathcal{D}}$ & $\mathcal{D}$ + $\hat{\mathcal{D}}$ \\
        \midrule
        None ($\hat{\mathcal{D}}$ = empty) & - & 64.4 & - & 65.6 & - & 72.0 \\
        \midrule
        \textit{Question Rewriting} & & & & & & \\
        \quad Back-translation & - & 63.4 & - & \textbf{67.7} & - & 70.8 \\
        \quad De-contextualization & - & 62.5 & - & 67.6 & - & 69.8 \\
        \midrule
        \textit{Single-turn QA Generation} & & & & & & \\
        \quad PAQ-CANARD & 38.2 & 64.3 & 38.8 & 66.5 & 37.5 & 71.5 \\
        \quad PAQ-QuAC & 44.9 & 59.8 & 47.1 & 62.1 & 42.7 & 65.8 \\
        \midrule
        \textit{Ours} & & & & & & \\
        \quad SimSeek-sym & 51.8 & 62.1 & 53.3 & 65.6 & 53.6 & 69.5 \\
        \quad SimSeek-asym & \textbf{62.5} & \textbf{65.3} & \textbf{64.8} & 67.6 & \textbf{71.5} & \textbf{73.1} \\
        \midrule \midrule
        \textit{Human Annotation ($\hat{\mathcal{D}}$ = QuAC$_\text{unseen}$)} & 65.3 & 67.5 & 65.0 & 70.3 & 72.3 & 73.8 \\
        \bottomrule
    \end{tabular}
    \end{threeparttable}
    \caption{Comparison over synthetic CQA generation methods based on the development set of QuAC in semi-supervised setup. We report F1 scores for the end CQA performance. First, models in each method are trained on labeled dataset $\mathcal{D}$. Then, synthetic CQA dataset $\hat{\mathcal{D}}$ is generated by the each method. Finally, student CQA models in varying size are fine-tuned on the datasets either $\hat{\mathcal{D}}$ or $\mathcal{D} + \hat{\mathcal{D}}$.}
    \label{table:semi_quac}
\end{table*}

==> archive/unseen_transpose_mod2.tex <==
\begin{table}[t]
    \small
    \centering
    \begin{threeparttable}
    \begin{tabular*}{\columnwidth}{llcc}
        \toprule
        \multirow{2}{*}{CQA Model} & Synthetic CQA & \multicolumn{2}{c}{Trained on} \\
        & generation & $\hat{\mathcal{D}}$ & $\mathcal{D}$ + $\hat{\mathcal{D}}$ \\
        \midrule
        \multirow{6}{*}{\rotatebox[origin=c]{90}{rota}} & \textit{Human} & \textit{65.3} & \textit{67.5} \\
        \cmidrule{2-4}
        & None & - & 64.4$^*$ \\
        & BT & - & 63.4$^*$ \\
        & Decon & - & 62.5$^*$ \\
        \cmidrule{2-4}
        & PAQ-CANARD & 38.2 & 64.3 \\
        & PAQ-QuAC & 44.9 & 59.8 \\
        & SimSeek-sym & 51.8 & 62.1 \\
        & SimSeek-asym & \textbf{62.5} & \textbf{65.3} \\
        % & + I-RTC & 62.7 & 65.1 \\
        \midrule
        \multirow{6}{*}{RoBERTa-large} & \textit{Human} & \textit{65.0} & \textit{70.3} \\
        \cmidrule{2-4}
        & None & - & 65.6$^*$ \\
        & BT & - & 67.7$^*$ \\
        & Decon & - & 67.6$^*$ \\
        \cmidrule{2-4}
        & PAQ-CANARD & 38.8 & 66.5 \\
        & PAQ-QuAC & 47.1 & 62.1 \\
        & SimSeek-sym & 53.3 & 65.6 \\
        & SimSeek-asym & \textbf{64.8} & \textbf{67.5} \\
        % & + I-RTC & \textbf{64.9}  & 67.6 \\
        \midrule
        \multirow{6}{*}{Longformer-large} & \textit{Human} & \textit{72.3} & \textit{73.8} \\
        \cmidrule{2-4}
        & None & - & 72.0$^*$ \\
        & BT & - & 70.8$^*$ \\
        & Decon & - & 69.8$^*$ \\
        \cmidrule{2-4}
        & PAQ-CANARD & 37.5 & 71.5 \\
        & PAQ-QuAC & 42.7 & 65.8 \\
        & SimSeek-sym & 53.6 & 69.5 \\
        & SimSeek-asym & \textbf{71.5} & \textbf{73.1} \\
        % & + I-RTC & 71.1 & - \\
        \bottomrule
    \end{tabular*}
    \end{threeparttable}
    \caption{Comparison over synthetic CQA generation methods based on QuAC development set (F1 score is reported) in semi-supervised setup. The $*$ indicates the CQA models do not take any synthetic dataset $\hat{\mathcal{D}}$, rather than rely on solely labeled dataset $\mathcal{D}$.}
    \label{table:semi_quac}
    \vspace{-3mm}
\end{table}

==> figs/data_analysis.tex <==
\begin{figure*}[t!] 
    \centering
    \includegraphics[width=1.0\textwidth]{imgs/synthetic_CQA_analysis_updated.png}
    \caption{Assessment of synthetic conversations upon three evaluation metrics. Specificity and informativeness are proposed by \citet{qi2020stay} to automatically evaluate the quality of generated questions. 
    In addition to those metrics, we further analyze answer relevance which checks the relevance of the answer with given conversational context. We find that the synthetic dataset from SimSeek-sym often too generic (low question specificity) and clearly obvious to be answered (high answer relevance) at the same time. However, we observe the human-annotated dataset (Original) shows moderate scores over all the metrics indicating some ambiguity is in the real scenario. On the other hand, the synthetic dataset from SimSeek-asym-L-large shows the most similar patterns with the human-annotated dataset.}
    \label{fig:data_analysis}
\end{figure*}

==> figs/nll_analysis.tex <==
\begin{figure}[t!] 
    \centering
    \includegraphics[width=\columnwidth]{imgs/question_ambiguity.png}
    \caption{Distributions of question ambiguity.}
    \label{fig:nll}
\end{figure}

==> tables/human_eval.tex <==
\begin{table}[t!]
\small
\centering
\resizebox{0.98\columnwidth}{!}{
\begin{tabular}{l|cccc}
    \toprule
     \multirow{2}{*}{Criterion} & \multicolumn{3}{c}{Judgement} & \multirow{2}{*}{$p$-value} \\
     & higher & neutral & lower & \\
    \midrule
    \midrule
    \multicolumn{5}{c}{\textbf{Asym vs. Sym}} \\
    \midrule
    Overall Adequacy & \textbf{0.42} & 0.25 & 0.34 & 0.086 \\
    Informativeness & 0.40 & 0.17 & 0.42 & 0.360 \\
    Context Relevance & 0.37 & 0.18 & 0.43 & 0.550 \\
    Answer Accuracy & 0.34 & 0.20 & \textbf{0.44} & 0.032 \\
    \midrule
    \multicolumn{5}{c}{\textbf{Asym vs. Human}} \\
    \midrule
    Overall Adequacy & \textbf{0.49} & 0.13 & 0.37 & 0.025 \\
    Informativeness & 0.40 & 0.17 & 0.43 & 0.354 \\
    Context Relevance & \textbf{0.39} & 0.27 & 0.34 & 0.024 \\
    Answer Accuracy & 0.36 & 0.28 & 0.37 & 0.448 \\
    \bottomrule
\end{tabular}}
\caption{Pairwise human evaluation results for the original QuAC (human) and the synthetic conversations from \textsc{SimSeek} (sym and asym). 
The annotators pick the better one from two random QA pairs in terms of each criterion.
We report the overall proportion of majority votes for each instance.
We conduct a bootstrap test with $10^5$ samples for the difference between pairs. 
Bold represents values with significant difference ($p$-value lower than 0.1).
}
\label{table:human_eval}
\vspace{-3mm}
\end{table}

==> tabs/04d_experimental_setup.tex <==
\section{Experimental Setup}

In this section, we specify our experimental setup and compare our frameworks to baseline approaches for generating CQA datasets. More implementation and experimental details are in Appendix~\ref{appendix:experimental_details},~\ref{appendix:implementation_details}.

\subsection{Datasets}

\paragraph{QuAC}

QuAC \cite{choi2018quac} consists of 100k QA pairs in information-asymmetric dialogues, where a questioner asks questions based on a topic with background information, and an answerer returns the answers in the form of text spans in Wikipedia document. 
Restricting the questioners from accessing the answer-containing document, the authors encourage them to seek new information on a topic via conversation. To simulate a semi-supervised setup, we split the original training set of QuAC into three subsets, QuAC$_{seen}$, QuAC$_{unseen}$, and the validation set\footnote{Subsets are partitioned following \citet{elgohary2019can}}. Detailed statistic is described in Table \ref{table:data_stat}.
Following \citet{choi2018quac}, we evaluate models with the F1 score for QuAC.
Since the test set is only available in the QuAC leaderboard, we evaluate models on the development set\footnote{\href{https://quac.ai/}{quac.ai}}.
We further detail the experimental setup in Appendix \ref{appendix:training_cqa}.


\paragraph{OR-QuAC}

\citet{qu2020open} extend the original QuAC dataset to open-domain setup\footnote{\href{https://github.com/prdwb/orconvqa-release}{github.com/prdwb/orconvqa-release}}. It assumes that a ground-truth document is not given in advance, which means the answerers do not know what to be asked before a conversation begins. 
Instead, they first need to search relevant passages from web-scale documents (about 11M chunked passages) based on the given conversational history and current question.
% Then, the answer to the input can be predicted based on the retrieved passages. 
After reading the retrieved passage, they predict an answer to the question.
Following the original setup in \citet{qu2020open}, we only regard previous questions $\{q_1, q_2, ..., q_{t-1}\}$ as history without answers. 
% Because of the setup, we can compare qualities of questions from our synthetic datasets aside from answers on OR-QuAC.
% % Hence, if backbone architecture is controlled, we can test how the given questions are relevant to the passage by evaluating the resulting models.
% we can compare qualities of questions from our synthetic datasets aside from answers on OR-QuAC.
Since OR-QuAC is similarly partitioned with our QuAC splits (see details in Table \ref{table:data_stat}), we use same synthetic conversations that are used for CQA task. More experimental details are in Appendix~\ref{appendix:or_quac}.
For evaluation, mean reciprocal rank (MRR), Recall@5 (R@5), and Recall@20 (R@20) are used to evaluate first stage conversational retrieval.


% \paragraph{Wikipedia Corpus}

\subsection{SimSeek for Semi-supervised Setup}

For semi-supervised CQA setup, we set QuAC$_{seen}$ as $\mathcal{D}$ and documents in QuAC$_{unseen}$ as $\mathcal{C}$. The number of turns $T$ is set to 6 in our generations.
%However, we utilize original QuAC train set as $\mathcal{D}$ and external Wikipedia corpus we collected as $\mathcal{C}$ for the full augmentation experiment.
For OR-QuAC experiment, we follow the semi-supervised setup since OR-QuAC shares the same document split with the semi-supervised setup. All CQG models are based on T5-large~\cite{raffel2020exploring} model, and we use 5 for beam size of beam search and 0.98 for top-$p$ value of nucleus sampling~\cite{holtzman2020curious} with 1.2 temperature. We employ the same backbone for the CAF with corresponding CQA student models, RoBERTa-base (R-base), RoBERTa-Large (R-large), and Longformer-large (L-large)~\cite{liu2019roberta, Beltagy2020Longformer}.
 
%HEQ measures whether a CQA model finds more accurate answers than humans in each granularirty (HEQ-Q for question, HEQ-D for dialogue). 

\subsection{Baselines for Synthetic CQA Generation}
We introduce strong baselines for synthesizing CQA datasets and compare them with our methods.
For a fair comparison, we train all components 
of approaches on the same labeled dataset $\mathcal{D}$, and generate the synthetic dataset $\hat{\mathcal{D}}$ on the unlabeled corpus $\mathcal{C}$.

\paragraph{Back-translation}
Back-translation is one of the most widely used methods for data augmentation in NLP fields~\cite{sennrich-etal-2016-improving, fadaee2017data, xie2020unsupervised}.
We translate an existing question $q$ from the labeled dataset $\mathcal{D}$ into another target language and then translate it back into the source language to obtain a paraphrased question. We set the target language as German (de) while the source language is English (en). 
Specifically, we use translation models for both directions (en -> de) and (de -> en), which are pre-trained on WMT-19~\cite{ng-etal-2019-facebook}.

\paragraph{De-contextualization}
\citet{elgohary2019can} rewrite conversational questions of QuAC into self-contained questions that could be understood without the conversation. 
Following \citet{kim2021learn}, we consider the resulting dataset, CANARD, as an additional dataset for training CQA models.
Note that CANARAD$_{train}$ and QuAC$_{seen}$ share the same passages.

\paragraph{PAQ-CANARD}
For the single-turn QA generation, \citet{lewis2021paq} propose PAQ, the pipeline strategy composed of three phases, answer extraction, question generation, and round-trip filtration.
Even though it is not designed to generate context-dependent questions, we generate de-contextualized conversations like CANARD~\cite{elgohary2019can}. 
Thus, we fine-tune every component of the PAQ on CANARD$_{train}$. Then, we include it as one of the baselines leveraging single-turn QA.
% For doing so, we fine-tune every component on CANARD$_{train}$.



% \subsection{Single-turn QA Generation}
% Recent studies for the synthetic QA generation propose the pipeline strategies composed of three sub-phases, answer extraction, question generation, and round-trip filtration \cite{alberti2019synthetic, puri2020training, lewis2021paq}.
% The first step, answer extraction, identifies spans in the given passage that are likely to be answer to question.
% An off-the-shelf tools for Named Entity Recognition (NER) or the trained answer extraction models are adopted for extracting answer candidates.
% % TODO: PLM 미리 약어쓰기
% For the next step, question generation, neural models for text generation are trained to generate coherent questions with the given answer and passage.
% % TODO: Answer-prior 를 활용하는 점 강조 
% Lastly, after generating synthetic $(q,a)$ pairs, a filtering QA model provides the predicted answer $\hat{a}$ given the generated question $q$.
% If the initial answer is not matched with the predicted one, the pair is discarded to ensure the round-trip consistency.

% These strategies have achieved remarkable success such that QA models trained on synthetic sets outperform them on the original training set.
% However, extending them to conversational setup is non-trivial.


\paragraph{PAQ-QuAC}

We construct a baseline by using a straightforward way to extend the single-turn QG framework, e.g., PAQ~\cite{lewis2021paq}, to a conversational setup.
We replace the question generator in PAQ with CQG$_{answer}$ model that also takes the conversation history as input. Different from our SimSeek-sym, the baseline utilizes the original answer extractor model of \citet{lewis2021paq}, which extracts answer candidates regardless of conversational history, i.e. $p_a(a \mid c)$. From a given answer-containing passage $c$, top-$k$ answer candidates are extracted by the model in advance. Then, we randomly take out an answer from the candidates to feed it to the CQG$_{answer}$ at every turns.

\input{tables/unseen}

\subsection{CQA Models}
After building synthetic CQA datasets upon the unlabeled corpus $\mathcal{C}$, the baseline CQA models are trained on the datasets.
By comparing the resulting CQA performances, we evaluate the effectiveness of the generated dataset $\hat{\mathcal{D}}$.
We test three backbone architectures for CQA, \texttt{base}
and \texttt{large} size of RoBERTa \cite{liu2019roberta}, and Longformer-\texttt{large} \cite{Beltagy2020Longformer}.
By contrasting various sizes of pre-trained models, we show the different effects of data augmentation.
In addition, we involve Longformer architecture that has been shown to be effective for encoding much longer history \cite{zhao2021ror}, which achieves competitive performance with the state-of-the-art approach.
% 이는 coherence of dialog를 보여줄것?


% \subsection{Implementation Details}



% \input{tables/unseen_seq}

% xxx



==> tabs/ethics.tex <==
\section*{Ethical Considerations}

\citet{choi2018quac} describe the limitations of QuAC dataset in their datasheet\footnote{\href{https://quac.ai/datasheet.pdf}{quac.ai/datasheet.pdf}}. 
QuAC might contain bias against famous people since articles were filtered on the ``people'' category associated with other subcategories of Wikipedia. 
Thus, the authors discourage model deployment trained on QuAC in real-world settings. Our \textsc{SimSeek} could be exposed to the same bias. However, we find \textsc{SimSeek} can generalize the category beyond ``people''. Table~\ref{table:case_study_ood} shows one of qualitative example in \textsc{Wiki-SimSeek}. Even if we argue the generalization ability relying on the qualitative results for now, we have a plan to investigate the topic in future work.

% \textsc{SimSeek-asym} successfully simulates conversations of unseen topics as well, even if it is trained on QuAC. Our dataset could be used for adapting unseen domains in CQA research.

==> tabs/xx_auto_analysis.tex <==
\section{Analysis and Discussion}
\label{sec:analysis}

\subsection{Assessment of Synthetic Dataset}
\input{figs/data_analysis}
\label{sec:assessment}


We further explore which factors determine the gain from synthetic conversations.
% Following \citet{lowe-etal-2017-towards, qi2020stay}, we investigate quantified qualities of synthetic conversations.
For quantifying the properties of question-answer pair, we adopt three metrics, question specificity, answer relevance, and answer informativeness, proposed by  \citet{lowe-etal-2017-towards, qi2020stay}. 
We train two additional classifier models. One is specificity classifier $p_s(q_t=\text{specific} \mid \mathcal{H}_t, q_t)$ to evaluate specificity of the synthetic questions as suggested by ~\citet{qi2020stay}. 
Another is answer relevance classifier $p_r(a_t=\text{relevance} \mid \mathcal{H}_t, q_t, a_t)$ judging relevance between conversational context and corresponding answer. 
We train the classifiers by contrasting negative examples. Specifically, frequent questions which appear more than once in the training dataset or random questions are sampled for the negative examples to train $p_s$ by 50\% of the time~\cite{qi2020stay}. To train $p_r$, we select random answers in the same conversation for the negatives by 50\% of the time. More implementation details are in Appendix~\ref{appendix:specificity_cls}. In addition to the two classifiers, we also adopt the informativeness metric proposed by \citet{qi2020stay}. It computes how much $a_t$ provides distinct and new information compared to previous answers $a_{1:t-1}$, i.e., $1 - \underset{1 \le i < t}{\max}\text{Precision}(a_t, a_i)$. It is another proxy to judge the usefulness of the corresponding question $q_t$.

Figure~\ref{fig:data_analysis} shows results of three metrics among various synthetic datasets and human-annotated dataset (Original). Especially, we plot the scores (y-axis) by conversational turns (x-axis) to get better understanding. First, we observe our SimSeek-asym datasets show similar patterns with the Original until 3rd turn in specificity (Figure~\ref{fig:data_analysis} (a)). However, the scores increase drastically as conversation progresses while the specificity of human questions increases slowly. In case of SimSeek-sym, it shows lower question specificity across all turns,  indicating that the questions are often generic, e.g. ``What else?'' or ``Anything else?''. Even though the general questions can be occurred naturally in information-seeking conversation, they make divergence of the conversation flow as discussed in \citet{qi2020stay}. The similar tendency is observed in Table~\ref{table:stat_comparison}. Actual percentage of the ``Anything else'' questions from SimSeek-sym is significantly higher than those of original QuAC and SimSeek-asym. Thus, keeping moderate specificity like Original is one of improvement points.

On the other hand, both answer relevance and informativeness show similar tendency. First, SimSeek-sym shows the highest answer relevance across all turns as shown in Figure~\ref{fig:data_analysis} (b). And it keeps its informativeness relatively high while informativeness scores of others continuously decrease (Figure~\ref{fig:data_analysis} (c)). It implies the answers of SimSeek-sym are clearly \textit{answerable} and the questions for them are less ambiguous which is far from realistic information-seeking. Actually, the number of unanswerable questions in SimSeek-sym are significantly less than others as shown in Table~\ref{table:stat_comparison}. Second, SimSeek-asym-L-large shows the most similar pattern with the Original in both answer relevance and informativeness. It implies that the synthetic questions and answers generated by SimSeek-asym-L-large mimic the realistic information-seeking conversation of human very well. However, when the RoBERTa-based model is used for the CAF, those two metrics decrease significantly as progress of conversation indicating importance of answerer, again.



% \subsection{Question Ambiguity}

% \input{figs/nll_analysis}

% We explore another way to quantify property of the synthetic questions in terms of ambiguity, Question Ambiguity. It is a simple idea leveraging answer-grounded CQG, CQG$_{answer}$. Specifically, we evaluate relationship of $(q_t, a_t)$ pair by quantifying how question $q_t$ is likely to be generated when answer $a_t$ is given. Formally, negative log likelihood of $q_t$ can be computed by CQG$_{answer}$, i.e. $-\log p_q^{sym}(q_t \mid c, a_t, \mathcal{H}_t)$ for the question ambiguity. For fair comparison, we train another CQG$_{answer}$ on the original QuAC training dataset instead of QuAC$_{seen}$. The question ambiguity scores from our two frameworks are illustrated in Figure~\ref{fig:nll}. As expected, SimSeek-asym shows long-tailed distribution with higher ambiguity compared to SimSeek-sym. The higher question ambiguity means the $q_t$ is not predictable from given $a_t$ and $\mathcal{H}_t$. In other word, the questions of SimSeek-asym tend to more open-ended and ambiguous, which contribute realistic information-seeking conversation.

% One might think the result of ambiguity conflict that of specificity in Section~\ref{sec:assessment}. However,

% We compare distributions of synthetic datasets to them of the original QuAC.
% For $(q,a)$ overlap, we count the number of matched tokens between question and answer at same turn.
% Same with Section \ref{sec:assessment}, we quantify overall scores  of informativeness and specificity, and count proportion of frequent questions (\% Frequent Qs).
% % Informativeness is measured by how many tokens newly appear in the current answer, compared to the conversation history.
% % The frequent questions are counted if same question text has appeared in the original QuAC (see details in Appendix~[ref]).

% As illustrated in Table \ref{table:stat_comparison}, the resulting dataset of SimSeek-sym significantly differs from the original QuAC dataset.
% In particular, SimSeek-sym generates dataset with high informativeness since CAE considers the previous answers when selecting current candidates.
% %  more frequently uses overlapped words with the answer.
% On the other hand, SimSeek-asym generates synthetic datasets whose statistics is more similiar with that of the original QuAC.
% Moreover, SimSeek-asym contains even smaller number of the frequent questions than annotators of QuAC, and asks more conversation-specific questions.


% Specifically, negative log likelihood (NLL) of $q_t$ can be computed by CQG$_{answer}$ which acts as a questioner in information-symmetric conversation~(Algorithm~\ref{algo:irtc}). We filter out questions from SimSeek-asym when their NLL exceeding specific threshold $\tau$. 

% Thus, evaluating QG performance with automatic lexical similarity (e.g., BLEU or ROUGE) could mislead to ...
% of synthetic questions can not guarantee improvement in CQA performance.
% We claim that ...
% Automatic evaluation =/= question 의 효용성 as data augmentation

% \subsection{Comparison of Synthetic CQA}
% \input{tables/stat_comparison}


